Parallel Wavelet Tree Construction

We present parallel algorithms for wavelet tree construction with polylogarithmic depth, improving upon the linear depth of the recent parallel algorithms by Fuentes-Sepulveda et al. We experimentally show on a 40-core machine with two-way hyper-threading that we outperform the existing parallel algorithms by 1.3--5.6x and achieve up to 27x speedup over the sequential algorithm on a variety of real-world and artificial inputs. Our algorithms show good scalability with increasing thread count, input size and alphabet size. We also discuss extensions to variants of the standard wavelet tree.

==> alg3.tex <==
\section{An $O(n\log\sigma/\sqrt{\log n})$ work parallel algorithm}
In this section, we discuss how to parallelize the
$O(n\log\sigma/\sqrt{\log n})$ work sequential wavelet tree
construction algorithm by Babenko et al.~\cite{BabenkoGKS14}.

We first describe how the sequential algorithm works.  The main idea
of the algorithm is to process integers of size smaller than
$\log\sigma$. The basic data structure is a \emph{packed list}, which
stores $N$ $b$-bit integers using $Nb/\log n$ words. It supports
appending a length $N$ list in $O(1+Nb/\log n)$ work and splitting a
list into smaller lists of at most length $k$ in $O(Nb/\log n + N/k)$
work. A \emph{big node} is defined to be a node at distance that is a
multiple of $\tau$ from the root, where $\tau$ is a parameter. Big
nodes store the elements that it represents in $\Str$, using
$\log\alpha$ bits per element as in the standard representation. These
can be computed recursively as follows. The root stores $\Str$. Assume
the sub-sequences for the big nodes at distance $\alpha\tau$ are
computed already. Then to compute the elements in the big nodes at
distance $(\alpha+1)\tau$, the big nodes at distance $\alpha\tau$ look
at the $\tau$ bits starting at position $\alpha\tau$ in the binary
representation of each element, to determine which of its descendant
big nodes at distance $(\alpha+1)\tau$ to place the element (there are
$2^\tau$ such descendants). The computation for big nodes requires
$O(n\log\sigma/\tau)$ work.

Babenko et al. make the observation that these nodes at all other
levels only need to store $\tau$ bits per element (the $\tau$ bits
starting at position $\alpha\tau$ where $\alpha\tau$ is the level of
its nearest big node ancestor) because there are only $\tau$ levels
between two big node levels.

These nodes use \emph{short lists} to store $\tau$-bit integers
containing the $\tau$ relevant bits of the elements it
represents. These are stored as packed lists.  Computing the bitmap
values and short lists can is done recursively. The short lists of the
children of a big node can be computed by extracting the relevant bits
from the elements of the big nodes in $O(n\log\sigma/\tau)$ work over
all big nodes. Given a short list of a node, computing its own bitmap
values and the short lists of its children is done via table look-up.
For all packed lists $L$ of at most length $\log n/(2\tau)$, the
bitmap value, and the packed lists $L_0$ and $L_1$ consisting of the
elements of $L$ whose $t$'th most significant bit is $0$ or $1$,
respectively are precomputed for all $t$ in $[0,\tau-1]$. Pre-computing
this table involves evaluating all $O(2^{\log n/(2\tau)})$ bit-strings
of length at most $\log n/(2\tau)$. Each node splits its short list
into blocks of length at most $\log n/(2\tau)$, performs table
look-ups for each block, and then appends the resulting bitmap values
together, $L_0$'s together and $L_1$'s together. The bitmap values are
stored in the bitmap associated with the current node, and $L_0$ and
$L_1$ are passed to its children.  For a node with a short list of
length $N$, the total work required is $O(N\tau/\log n)$ as the
splitting and merging can be done in $O(N\tau/\log n)$ work overall
and table look-ups in constant work per block.  The lengths of all
short lists is $O(n\log\sigma)$, so the total work required for this
computation is $O(n\log\sigma\tau/\log n)$.

The overall work is $O(n\log\sigma/\tau + n\log\sigma\tau/\log n)$ and
by choosing $\tau = \sqrt{\log n}$, the work is
$O(n\log\sigma/\sqrt{\log n})$.

We now discuss how to parallelize the algorithm. We will assume that
$\tau$ has been chosen to be $\sqrt{\log n}$. A bitmap is stored per
node, instead of per level, as computed the offsets in parallel into
the level bitmaps would require a prefix sum per level, leading to
$O(\sigma\log\sigma)$ work, which is too expensive for large $\sigma$.
 
The sub-sequences for the big nodes can be computed level-by-level
using integer sorting. In particular, given the correct sub-sequence
$\Str'$ for a big node at level $\alpha\sqrt{\log n}$, we compute the
sub-sequences for its big node descendants at level
$(\alpha+1)\sqrt{\log n}$ by performing integer sort on $\Str'$, where
the key is the $\sqrt{\log n}$ bits starting from position
$\alpha\sqrt{\log n}$. The integer sort requires linear work and
$O(\log n)$ span per level, and over the $\log\sigma/\sqrt{\log n}$
levels, this gives $O(n\log\sigma/\sqrt{\log n})$ work and
$O(\sqrt{\log n}\log\sigma)$ span.

The table for queries can be precomputed by evaluating all
$O(2^{\sqrt{\log n}/2})$ bit-strings of length at most $\sqrt{\log
  n}/2$ in parallel, and storing the answer for each in a unique
location.  Each bit-string is evaluated sequentially. Overall, this
requires $O(\sqrt{\log n})$ span and $o(n)$ work. 

Computing short lists for children of a big node can be done in linear
work and $O(\log n)$ span using prefix sums. Computing short lists
other nodes requires merging and splitting packed lists. For a short
list of length $N$, we split it into chunks of length at most
$\sqrt{\log n}/2$ by copying the relevant bits of each chunk into its
own word in constant span. All look-ups into the table are done in
parallel in constant span. To merge the results together, we compute
the length (in bits) of each result, perform a prefix sum to determine
the total length (in bits) and also the offset for each result in a
new array, allocate a new array of the desired length, and then copy
each result into the new array in parallel. Since the results are
smaller than a word, the copy is performed atomically using a
compare-and-swap loop. This requires $O(N/\sqrt{\log n})$ work if the
short list contains $N$ integers, since the integers are represented
using only $\sqrt{\log n}$ bits.  The overall work for computing the
short lists is $O(n\log\sigma/\sqrt{\log n})$ as in the sequential
algorithm.  The span is $O(\log n\log\sigma)$ as there are
$\log\sigma$ levels, each requiring $O(\log n)$ span.

We obtain the following theorem:
\begin{theorem}
Wavelet tree construction can be performed in
$O(n\log\sigma/\sqrt{\log n})$ work and $O(\log n\log\sigma)$ span.
\end{theorem}

The algorithm has a peak memory usage of $O(n\log n)$ bits due to the
prefix sum, which is higher than the space bound of $O(n\log\sigma)$
bits for the sequential algorithm.


==> implementation.tex <==
\section{Implementation}
Describe optimization with atomic OR. Times for construction with and
without tree pointers.

